Fast discovery of multidimensional subsequences for robust trajectory classification

Trajectory classification tasks became more complex as large volumes of mobility data are being generated every day and enriched with new sources of information, such as social networks and IoT sensors. Fast classification algorithms are essential for discovering knowledge in trajectory data for real applications. In this work we propose a method for fast discovery of subtrajectories with the reduction of the search space and the optimization of the MASTERMovelets method, which has proven to be effective for discovering interpretable patterns in classification problems.

==> sections/0_1_Definitions.tex <==
%%%% DEFINITIONS / NOMENCLATURE %%%%
\newcommand{\hm}{HiPer Movelets}

\newcommand{\HM}{HiPerMovelets}
\newcommand{\HML}{\HM{}-Log}
\newcommand{\HP}{\HM{}-Pivots}
\newcommand{\HPL}{\HP{}-Log}

\newcommand{\M}{Movelets}

\newcommand{\MM}{MASTERMovelets}
\newcommand{\MML}{\MM{}-Log}

\newcommand{\SM}{SUPERMovelets}
\newcommand{\SML}{SUPERMovelets-Log}
\newcommand{\MP}{MASTERPivots}
\newcommand{\MPL}{MASTERPivots-Log}


% \newenvironment{CL}
% {\color{red!50!black}}
% {\color{black}}

% \newenvironment{TP}
% {\color{lime!20!black}}
% {\color{black}}

\newcommand{\mr}[2]{\multirow{#1}{*}{#2}}

\DeclareMathOperator{\Tparam}{0.5}
\DeclareMathOperator{\Tparamper}{50\%}

\newcommand{\bl}[1]{\textbf{#1}}
\newcommand{\un}[1]{\underline{#1}}

% COLORING CMDs
% \newcommand{\x}[1]{\textcolor{purple}{#1}}
% \newcommand{\y}[1]{\textcolor{red!50!black}{#1}}
% \newcommand{\V}[1]{\textcolor{blue}{VB: #1}}
% \newcommand{\T}[1]{\textcolor{green!40!black}{TP: #1}}
% \newcommand{\Ts}[1]{\T{\st{#1}}}
% \newcommand{\Vs}[1]{\V{\st{#1}}}

% NO - COLORING CMDs
\newcommand{\x}[1]{#1}
\newcommand{\y}[1]{#1}
\newcommand{\V}[1]{}
\newcommand{\T}[1]{}
\newcommand{\Ts}[1]{}
\newcommand{\Vs}[1]{}

\renewcommand{\imprimirpreambulo}{%
Thesis submitted to the 
\imprimirprograma{} for the degree of Doctor of Philosophy.%
}

==> sections/0_Imports.tex <==
% \usepackage[T1]{fontenc} % fontes
\usepackage[utf8]{inputenc} % UTF-8
\usepackage{pdfpages} % Inclui PDF externo (ficha catalográfica)
% \usepackage{multirow}
\usepackage{colortbl} 
\usepackage{subcaption}
\usepackage{soulutf8}
\usepackage{color}
\usepackage{parskip}

\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{caption}
\usepackage{xcolor}

\usepackage{algorithm}
\usepackage[noend]{algpseudocode}

\usepackage{multirow}
\usepackage{lipsum,booktabs}

\usepackage[normalem]{ulem}

\usepackage{mathtools}
% \usepackage{amsmath}
% \usepackage{amsthm}
\usepackage{amssymb,amsmath,amsthm}
\usepackage{amsfonts}
% \usepackage[mathscr]{eucal}
% \usepackage[mathcal]{eucal}
% \usepackage{mathrsfs}
\DeclareSymbolFont{cmsymbols}{OMS}{cmsy}{m}{n}
\SetSymbolFont{cmsymbols}{bold}{OMS}{cmsy}{b}{n}
\DeclareSymbolFontAlphabet{\mathcal}{cmsymbols}

\newcommand{\argmax}{\mathop{\textit{argmax}}\limits}
% \DeclareMathOperator*{\argmax}{argmax}

\usepackage{pdflscape}
\usepackage{subcaption}
\usepackage{array}
\newcommand{\PreserveBackslash}[1]{\let\temp=\\#1\let\\=\temp}
\newcolumntype{C}[1]{>{\PreserveBackslash\centering}p{#1}}
\newcolumntype{L}[1]{>{\PreserveBackslash\raggedright}p{#1}}
\newcolumntype{R}[1]{>{\PreserveBackslash\raggedleft}p{.15\textwidth}|}
% ----------------------------------------------------------
\usepackage{nomencl}
\makenomenclature

%MAKE DEFINITIONS
\theoremstyle{definition}
\newtheorem{definition}{Definition}

% LIST OF SYMBOLS
% -------------------------------------------------------------
\renewcommand{\nomname}{List of Symbols}
\setlength{\nomitemsep}{0.0em}

% Macro para que apareçam na ordem em que forma definidos
\providetoggle{nomsort}
\settoggle{nomsort}{true}
\makeatletter
\iftoggle{nomsort}{%
    \let\old@@@nomenclature=\@@@nomenclature        
        \newcounter{@nomcount} \setcounter{@nomcount}{0}%
        \renewcommand\the@nomcount{\two@digits{\value{@nomcount}}}% Ensure 10>01
        \def\@@@nomenclature[#1]#2#3{% Taken from package documentation
          \addtocounter{@nomcount}{1}%
        \def\@tempa{#2}\def\@tempb{#3}%
          \protected@write\@nomenclaturefile{}%
          {\string\nomenclatureentry{\the@nomcount\nom@verb\@tempa @[{\nom@verb\@tempa}]%
          \begingroup\nom@verb\@tempb\protect\nomeqref{\theequation}%
          |nompageref}{\thepage}}%
          \endgroup
          \@esphack}%
      }{}
\makeatother
